GuardT2I: Defending Text-to-Image Models from Adversarial Prompts

Recent advancements in Text-to-Image (T2I) models have raised significant safety concerns about their potential misuse for generating inappropriate or Not-Safe-For-Work (NSFW) contents, despite existing countermeasures such as NSFW classifiers or model fine-tuning for inappropriate concept removal. Addressing this challenge, our study unveils GuardT2I, a novel moderation framework that adopts a generative approach to enhance T2I models' robustness against adversarial prompts. Instead of making a binary classification, GuardT2I utilizes a Large Language Model (LLM) to conditionally transform text guidance embeddings within the T2I models into natural language for effective adversarial prompt detection, without compromising the models' inherent performance. Our extensive experiments reveal that GuardT2I outperforms leading commercial solutions like OpenAI-Moderation and Microsoft Azure Moderator by a significant margin across diverse adversarial scenarios. Our framework is available at https://github.com/cure-lab/GuardT2I.

==> sec/3_problem_statement.tex <==
\section{Problem Statement}
\label{sec:problem_statement}
In this section, we first specify the threat model adopted in this paper, which includes the targets and capabilities of both adversaries and defenders.
Then, we present our design goals and the research challenges associated with them, which are our major motivations for designing new moderation methods.


\subsection{Threat Model}
\noindent\textbf{Attacker's Target and Capability.}
Given a T2I system, we consider potential attackers targeting to generate inappropriate content (\ie, image) by designing or collecting prompts (\ie, text) that guide the T2I generation.
Inappropriate content includes various concepts but is not limited to \texttt{violent}, \texttt{pornographic}, and \texttt{gore} themes.
Besides, adversarial attackers have access to some open-source T2I models, such as SD~\cite{sdcheckpoint}.
Both manual or automatic attacking methods are allowed, as in Section~\ref{sec:related_attacks}.
Further, they are aware of the existence of simple prompt filters that reject prompts containing sensitive words~\cite{mma}. 

\noindent\textbf{Defenders' Target and Capability.} In this paper, we propose a prompt-based content moderator, whose target is to identify malicious prompts and reject them from T2I systems, where malicious prompts are those that lead to syntheses with inappropriate images.
Such a defender only has access to the provided prompt and the T2I system in use, while has no knowledge about the attackers (\eg, the construction process of adversarial prompts).
Besides, the defensive method should not reject benign prompts or reject only a few of them.


\subsection{Research Goals and Challenges}\label{sec:goal-challenges}

Our research focuses on addressing the critical challenge of ensuring the safety of T2I models against adversarial prompts intended to generate inappropriate content. The following goals outline the scope and direction of our efforts:

\noindent \circled{1} \textbf{Attack-agnostic design}: We aim to design an attack-agnostic moderation framework capable of responding to a variety of adversarial prompts. This framework should exhibit stable performance across different attack methodologies or malicious prompts.

\noindent \circled{2} \textbf{Scalability to various appropriate content.} It is hard to formally define all inappropriate content at once, and the exact type of content may vary through time and geographical conditions. The defensive framework should be flexible and dynamic, capable of rapidly adapting to new content.

\noindent\circled{3} \textbf{Seamless integration with T2I models}: The defensive methods should have little or no influence on the generation of benign content. This goal ensures that the inherent performance, along with the quality and diversity of the generated images, remains unaffected.

\noindent \circled{4} \textbf{Interpretability for decision-making}: It would be better if defensive methods provide possible reasons why an input prompt is rejected.
This feature can enhance the user experience of the T2I system, while also making it easier for developers to identify intentions behind malicious prompts and understand misjudgment issues. 


Currently, no other literature or system is resolving all four challenges.
In this work, we mainly focus on \circled{1}-\circled{3}, which is more crucial to mitigating the threats from malicious prompts.
Besides, we make a preliminary attempt to meet \circled{4}.
By focusing on these research goals, we aim to establish a novel moderation paradigm for the content safety of T2I models, ensuring that T2I models can be utilized in a safe, responsible, and ethically sound manner.
